No Reservations: A First Look at Amazon's Reserved Instance Marketplace

Cloud users can significantly reduce their cost (by up to 60\%) by reserving virtual machines (VMs) for long periods (1 or 3 years) rather than acquiring them on demand. Unfortunately, reserving VMs exposes users to \emph{demand risk} that can increase cost if their expected future demand does not materialize. Since accurately forecasting demand over long periods is challenging, users often limit their use of reserved VMs. To mitigate demand risk, Amazon operates a Reserved Instance Marketplace (RIM) where users may publicly list the remaining time on their VM reservations for sale at a price they set. The RIM enables users to limit demand risk by either selling VM reservations if their demand changes, or purchasing variable- and shorter-term VM reservations that better match their demand forecast horizon. Clearly, the RIM's potential to mitigate demand risk is a function of its price characteristics. However, to the best of our knowledge, historical RIM prices have neither been made publicly available nor analyzed. To address the problem, we have been monitoring and archiving RIM prices for 1.75 years across all 69 availability zones and 22 regions in Amazon's Elastic Compute Cloud (EC2). This paper provides a first look at this data and its implications for cost-effectively provisioning cloud infrastructure.

==> discussion.pradeep.tex <==
We believe that our paper is one of the first work to analyze the AWS Reserved Instance Marketplace (RIM) data. We present first look of the RIM by presenting its high level details (and insights) like total market volume over time, comparison of all EC2 regions by average market volume, top instance types etc. In other words, we present macro analysis of the marketplace and there are many other insights that can be analyzed. In particular, we can look at the several micro details. For example:

\begin{itemize}
  \item What is the mean time to sell an instance in RIM? What factors affect this mean time?
  \item Does market volume fluctuates by seasonal effects e.g., holiday season?
  \item How to set the instance price given the duration, offering type, and region etc.?
\end{itemize}

% In this work, we present analysis from a third person perspective. It would be interesting to analyze the data from both the buyers and sellers perspective. Buyers and sellers have different priorities when its to using the RIM as buyers prefer to get the instances for cheaper price whereas sellers might prefer to sell at an profit and in a faster time as well. 

By opensourcing the RIM data, we expect to generate interesting discussions at the workshop and gives opportunity to analyze the data for indepth analysis of marketplace. One of the first points of discussion could be does RIM benefit buyers or sellers or platform itself? We expect with mature regions (markets) RIM can benefit all of the parties, as RIM allows users to sell their unused instances and at the same time RIM allows users buy the reserved instances with less than 1 year (or 3 year) reservation as well. So, users can strategically buy the reserved instances (and at the later time can sell the reserved instances) to cost-effectively provisioning cloud infrastructure. 

% Another point of discussion, can users use RIM for extending or not paying for thier reservation during the idle periods? For example users can list their reservation for very high price and later cancel the listing, so that they avoid paying for the reservation during the listing time and still retain the same term limit as just before the listing being floated in RIM.

==> evaluation.tex <==
blah
